Development of End-to-End Low-Cost IoT System for Densely Deployed PM Monitoring Network: An Indian Case Study

Particulate matter (PM) is considered the primary contributor to air pollution and has severe implications for general health. PM concentration has high spatial variability and thus needs to be monitored locally. Traditional PM monitoring setups are bulky, expensive and cannot be scaled for dense deployments. This paper argues for a densely deployed network of IoT-enabled PM monitoring devices using low-cost sensors. In this work, 49 devices were deployed in a region of the Indian metropolitan city of Hyderabad out-of this, 43 devices were developed as part of this work and 6 devices were taken off the shelf. The low-cost sensors were calibrated for seasonal variations using a precise reference sensor. A thorough analysis of data collected for seven months has been presented to establish the need for dense deployment of PM monitoring devices. Different analyses such as mean, variance, spatial interpolation and correlation have been employed to generate interesting insights about temporal and seasonal variations of PM. In addition, event-driven spatio-temporal analysis is done for PM values to understand the impact of the bursting of firecrackers on the evening of the Diwali festival. A web-based dashboard is designed for real-time data visualization.

==> Backup.tex <==
The specific contributions of this paper are:
\begin{enumerate}
    \item For precise monitoring of outdoor PM, 49 IoT-based PM monitoring device has been developed, calibrated and deployed at various outdoor locations.
    \item A robust IoT-based PM monitoring device has been developed, which is foolproof against the issue of data loss due to connection and power outages as it maintains an offline cache. The stored data is offloaded in bulk, once the power and communication is restored. All 49 PM sensors calibrated for seasonal variations by co-locating with a reference sensor.
   \item The devices were deployed at 49 outdoor locations covering a $4\, \text{km}^2$ area in Gachibowli, Hyderabad, India. The field locations were selected to include urban, semi-urban, and green regions. Few devices were deployed at busy traffic junctions and roadsides. The data was recorded at a frequency of every 30 seconds (sec) spanning over all the seasons for six months, thus aggregating 14.23 million data points.
   \item A web-based dashboard has been developed to visualize the data in real-time. 
   \item Analysis like correlation, seasonal variation and Diwali effect has been done. Correlation analysis has been carried out to find the impact of local activities on PM and establish the necessity of dense deployment. The effects of seasonal variations and the Diwali festival on PM were analyzed using time series plots and the inverse distance weighting interpolation technique. Results obtained showed the optimal deployment across a varied landscape and can be a key factor in identifying high concentration release of PM.
\end{enumerate}

